Intersectional Affirmative Action Policies for Top-k Candidates Selection

We study the problem of selecting the top-k candidates from a pool of applicants, where each candidate is associated with a score indicating his/her aptitude. Depending on the specific scenario, such as job search or college admissions, these scores may be the results of standardized tests or other predictors of future performance and utility. We consider a situation in which some groups of candidates experience historical and present disadvantage that makes their chances of being accepted much lower than other groups. In these circumstances, we wish to apply an affirmative action policy to reduce acceptance rate disparities, while avoiding any large decrease in the aptitude of the candidates that are eventually selected. Our algorithmic design is motivated by the frequently observed phenomenon that discrimination disproportionately affects individuals who simultaneously belong to multiple disadvantaged groups, defined along intersecting dimensions such as gender, race, sexual orientation, socio-economic status, and disability. In short, our algorithm's objective is to simultaneously: select candidates with high utility, and level up the representation of disadvantaged intersectional classes. This naturally involves trade-offs and is computationally challenging due to the the combinatorial explosion of potential subgroups as more attributes are considered. We propose two algorithms to solve this problem, analyze them, and evaluate them experimentally using a dataset of university application scores and admissions to bachelor degrees in an OECD country. Our conclusion is that it is possible to significantly reduce disparities in admission rates affecting intersectional classes with a small loss in terms of selected candidate aptitude. To the best of our knowledge, we are the first to study fairness constraints with regards to intersectional classes in the context of top-k selection.

==> removed.tex <==
%!TEX root = main.tex

\clearpage\appendix
\section{Removed from introduction (repetitive)}

To make our work more concrete and easier to understand, throughout this paper we will look at university admission policies. In many university systems, students who want to apply for undergraduate programs are required to present their high school grades and to take some standardized tests. The idea behind is that these quantities well predict a candidate's aptitude for tertiary education and his - her future performance. Admission rankings are therefore created using a weighed linear combination of both high school grades and standardized tests results.

...

For example, let's assume that in our pool of applicants rich white men had admission scores persistently higher than any other intersectional group. In this scenario, our methodology would avoid delivering a final ranking made up only of students from this specific group. In fact, discrepancies between the system acceptance rate and any other intersectional class admission rate would heavily penalize the final value of the solution found. It follows that optimizing the process with respect to our method induces a mechanism that would reward disadvantaged groups in order to decrease discrepancies.

Looking at the university system as a whole, our experiments clearly show that it is possible to admit students from all intersectional classes at a comparable rate, without a significant drop in the system total utility. This remains true even when there are large differences between groups admission score distributions.

\subsection{Linear Programming Approach}

As shown in box \ref{box:LPF}, our problem can be formulated as an integer linear program.

\medskip
\begin{framed}
\label{box:LPF}
Relaxed Linear program for  the Fair Set Cover problem:
$$
\begin{cases}
max \quad \displaystyle \sum_{i \in \textbf{C}} b_i - c_i &\\
s.t. \quad \displaystyle \sum_{s \in C_i} u_sx_s = b_i \quad & \forall C \in \textbf{C} \\
and \quad c_i \geq p - \frac{\sum_{s \in C_i} x_s}{\mid C_i \mid} & \forall C \in \textbf{C} \\
and \quad  c_i \geq \frac{\sum_{s \in C_i} x_s}{\mid C_i \mid} -p & \forall C \in \textbf{C} \\
and \quad \sum_i \sum_{s \in C_i} x_s = k & \\
\end{cases}
$$
Where $u_s$ represents student $s$ admission score, $x_s$ is an indicator function that tells whether student s will be admitted or not, $b_i$ is the total utility of admitted students from intersectional class $C_i$, and $c_i$ its discrepancy with respect to admission rate $p$.
\end{framed}
\medskip

\spara{Analysis.} Since integer linear programming problems can not be solved to the optimum in polynomial time, we relaxed the integrality constraint, allowing $x_s$ variables to range between 0 and 1. Consequently, the set of admitted students will be made up of the top $p\%$ of all applicants.

